On the Monitoring of Decentralized Specifications Semantics, Properties, Analysis, and Simulation

We define two complementary approaches to monitor decentralized systems. The first relies on those with a centralized specification, i.e, when the specification is written for the behavior of the entire system. To do so, our approach introduces a data-structure that i) keeps track of the execution of an automaton, ii) has predictable parameters and size, and iii) guarantees strong eventual consistency. The second approach defines decentralized specifications wherein multiple specifications are provided for separate parts of the system. We study two properties of decentralized specifications pertaining to monitorability and compatibility between specification and architecture. We also present a general algorithm for monitoring decentralized specifications. We map three existing algorithms to our approaches and provide a framework for analyzing their behavior. Furthermore, we introduce THEMIS, a framework for designing such decentralized algorithms and simulating their behavior. We show the usage of THEMIS to compare multiple algorithms and verify the trends predicted by the analysis by studying two scenarios: a synthetic benchmark and a real example.

==> alg-choreography.tex <==
\subsection{Choreography}
Choreography splits the initial LTL formula into subformulae and delegates each subformula to a monitor on a component.
Thus choreography can illustrate how it is possible to monitor decentralized specifications.
Recall from the definition of $\Delta'$ (see \rdef{def:sem-decent}), that monitoring is recursively applied to the remainder of a trace starting at the current event.
That is, initially we monitor from $e_0$ to $e_n$ and then from $e_1$ to $e_n$ and so forth.
To do so, it is necessary to reset the state of a monitor appropriately, we call this process a \emph{respawn}. 
In this section, we present first the generation of the decentralized specification from the LTL formula.
Then we illustrate how the network of monitors is setup.
And finally we present the monitoring algorithm applied for each monitor.


~

Choreography begins by taking the main formula, then deciding to split it into subformulae.
Each monitor will monitor the subformula, notify other monitors of its verdict, and when needed \emph{respawn}.
Once the subformulae are determined, we generate an automaton per subformula to monitor it.
Then, we construct the network of monitors in the form of a tree, in which the root is the main monitor.
Verdicts for each subformula are then propagated in the hierarchy until a verdict can be reached by the root monitor.

A choreography monitor is a tuple $\tuple{id,\aut_{\varphi_{id}}, \chorref_{id}, \chorcoref_{id}, \chorresp_{id}}$ where:
\begin{itemize}
	\item $id$ denotes the monitor unique identifier (label);
	\item $\aut_{id}$ the automaton that monitors the subformula;
	\item $\chorref_{id} : 2^{\mons}$ the monitors that this monitor should notify of a verdict;
	\item $\chorcoref_{id} : 2^{\mons}$ the monitors that send their verdicts to this monitor;
	\item $\chorresp_{id} : \verdictb$ specifies whether the monitor should \emph{respawn};
\end{itemize}
To account for the verdicts from other monitors, the set of possible atoms is extended to include the verdict of a monitor identified by its id. 
Therefore, $\atoms = (\timestamp \times \AP) \cup (\mons \times \timestamp)$.
Monitoring is done by replacing the subformula by the id of the monitor associated with it.


Before splitting a formula, it is necessary to determine the component that hosts its monitor.
We compute a component score by counting the number of atomic propositions associated with a component in the subformula.
\begin{align*}
\scor(\varphi, c) 
				&: LTL \times \comps \rightarrow \timestamp\\
				&= \texttt{ match $\varphi$ with }\\
				 & \begin{array}{ll}
				\mid a \in AP 				  & \rightarrow \twopartdef{1}{\clookup(a) = c} {0} \\
				\mid \text{ op } \phi	 	  & \rightarrow \scor(\phi, c)\\
				\mid \phi \text{ op } \phi'	  & \rightarrow \scor(\phi, c) + \scor(\phi', c)\\
\end{array}
\end{align*}
The chosen component is determined by the component with the highest score, using $\cchoose : LTL \rightarrow \comps $:
\[
	\cchoose(\varphi) = \underset{c \in \comps}{\operatorname{arg max}}  (\scor(\varphi, c)) 
\]

In order to setup the network of monitors, firstly the LTL expression is split into subformulae and the necessary monitors are generated to monitor each subformula.
The tree of monitors is generated by recursively splitting the formula at the binary operators.
Given the two operands, we choose which operands remains in the host component, and (if necessary) which would be placed on a different component.
Therefore, we add the constraint that at least one part of the LTL expression must still remain in the same component.
Given two formulas $\varphi$ and $\varphi'$ and an initial base component $c_{b}$ we determine the two components that should host $\varphi$ and $\varphi'$ with the restriction that one of them is $c_{b}$:
\begin{align*}
	c_1 = \cchoose(\varphi) &, \quad c_2 = \cchoose(\varphi')\\
	s_1 = \scor(\varphi, c_b) &, \quad s_2 = \scor(\varphi', c_b)\\
	\csplit(\varphi, \varphi', c_b)  
							 & = \funcparts{
		\tuple{c_b, c_b} & \pif c_1 = c_2 = c_b \\
		\tuple{c_1, c_b} & \pif (c_1 \neq c_b) \land (c_2 = c_b \lor s_2 > s_1)\\
		\tuple{c_b, c_2} & \pelse 	
}
\end{align*}
\ralg{alg:choreography-setup} displays the procedure to split the formula.
For each binary operator, we determine which of the operands needs to be hosted in a new component.
The result is a tuple: $\tuple{root, N, E}$ where:
\begin{itemize}
	\item $root$ is the root of the tree;
	\item $N$ is the set of generated monitor data;
	\item $E$ is the set of edges between the monitors.
\end{itemize}
Monitor data is a pair $\tuple{id, spec}$ that represents the id of the monitor and the formula that it monitors.

\begin{itemize}
	\item First, $\cchoose$ determines the $\vars{host}$ component where the root monitor resides.
	\item Second, the AST of the $LTL$ formula is traversed using $\func{netx}$, which splits on binary operators. 
		\begin{itemize}
			\item If both formulae can be monitored with the same monitor it does not split.
			\item Otherwise
			\begin{enumerate}
				\item We recurse on the side kept, to further split the formula;
				\item We recurse on the side split, with a new $host$ and $id$;
				\item We merge the subnetworks by:
					\begin{enumerate}
						\item Generating the host monitor with the formula resulting from the recursion;
						\item Connecting the split branch's root monitor to the current host monitor;
						\item Adding the split branch's root monitor to the set of additional monitors;
						\item Merging the set of additional monitors and edges from both branches.
					\end{enumerate}
			\end{enumerate}
		\end{itemize}
\end{itemize}


\begin{algorithm}[!tp]
 \caption{Setting up the monitor tree}
 \label{alg:choreography-setup}
\begin{algorithmic}[1]
	\Procedure{$NET\_CHOR$}{$\varphi, C, M$}
		\State $id \gets 0$
		\State $c_h \gets \cchoose(\varphi)$
		\State $\tuple{root, mons, edges} \gets netx(\varphi, id, c_h)$
		\State \Return $\tuple{\setof{root} \cup mons, edges}$
	\EndProcedure
	\Procedure{$netx$}{$\varphi, id_c, c_h$}
		\If{$\varphi \in AP$}
			\State $m \gets \tuple{\varphi, id_c}$
			\State \Return $\tuple{m, \emptyset, \emptyset}$
		\ElsIf{$\varphi$ matches op $e$} \Comment{Unary Operator}
			\State $o \gets \func{netx}(e, id_c, c_h)$
			\State $m \gets \tuple{\mbox{op } o.f, id_c}$
			\State \Return $\tuple{m, o.N, o.E}$
		\ElsIf{$\varphi$ matches $e$ op $e'$}
			\State $\tuple{c_1, c_2} \gets split(e, e', c_h, M)$
			\If{$c_1 = c_2 = c_h$} \Comment{No Split}
				\State $l \gets netx(e, id_c, c_h)$
				\State $r \gets netx(e', id_c, c_h)$
				\State $m \gets \tuple{l.f \mbox{ op } r.f, id_c}$
				\State \Return $\tuple{m, l.N \cup r.N, l.E \cup r.E}$
			\ElsIf{$c_1 = c_h$} \Comment{Split Right Branch}
				\State $id_n \gets \func{newid}()$
				\State $l \gets netx(e , id_c, c_h)$
				\State $r \gets netx(e', id_n, c_2)$
				\State $m \gets \tuple{l.f \mbox{ op } \tuple{id_n}, id_c}$
				\State \Return $\tuple{m, (l.N \cup r.N \cup {r.root}),(l.E \cup r.E \cup \setof{\tuple{id_n, id_c})} }$
			\Else \Comment{Split Left Branch}
				\State $id_n \gets \func{newid}()$
				\State $l \gets netx(e , id_n, c_1)$
				\State $r \gets netx(e', id_c, c_h)$
				\State $m \gets \tuple{\tuple{id_n} \mbox{ op } r.f, id_c}$
				\State \Return $\tuple{m, (l.N \cup r.N \cup {l.root}),(l.E \cup r.E \cup \setof{\tuple{id_n, id_c}}) }$
			\EndIf
		\EndIf
	\EndProcedure
\end{algorithmic}
\end{algorithm}

Once the monitor data tree is created, monitors are created accordingly, generating an automaton for the subformula, where some of its atomic propositions have been replaced with monitor ids.
Each monitor is initialized with the refs and corefs set based on the edges setup.

\begin{remark}[Compacting the network]
The monitor network can further be compacted as follows; monitors with the same subformula are merged into one, and their refs and corefs will be the result of the set union.
However one or more merged monitor will have to replace all occurence of the id of the other monitors in all subformulae of all monitors.
\end{remark}

The state of the choreography monitor consists of a tuple: $\tuple{t_\mathrm{mon}, \mem, \sys, \chorkill}$.
\begin{itemize}
	\item $t_\mathrm{mon}$ specifies the timestamp this monitor is monitoring;
	\item $\mem$ the memory of the monitor;
	\item $\sys$ is the $\MemRep{}$ encoding of the execution of $\aut_{id}$;
	\item $\chorkill \subseteq \chorref$ specifies the monitors that no longer require the verdict of this monitor;
\end{itemize}
The messages exchanged while monitoring are the following:
\begin{itemize}
	\item $\msgkill(id)$: indicates that the monitor $id$ no longer depends on the verdict of the monitor;
	\item $\msgverdict(id, t, v)$: indicates that the monitor $id$ has reached a verdict $v$ for timestamp $t$.
\end{itemize}




Monitoring is shown in \ralg{alg:choreography-monitor}, each monitor is monitoring a subformula for a specific timestamp.
The monitoring procedure begins by merging the observations with the memory, then in checking for received messages.
\begin{itemize}
	\item Upon receiving a $\msgkill(id_{\mathrm{from}})$, the monitor updates the $\chorkill$ set by adding $id_{\mathrm{from}}$, then checks if $\chorkill = \chorref$, if they are equal then no more monitors depend on the verdicts of this monitor, and if it is killed; i.e., it stops monitoring.
	\item Upon receiving a $\msgverdict(id_{\mathrm{from}}, t_v, v)$, where $v \in \verdictb$, it updates its memory as follows: $\mem := \mem \memadd [\tuple{t_v, id_{\mathrm{from}}} \mapsto v]$. This allows its corresponding atom ($\tuple{t_v, id_{\mathrm{from}}}$) to be evaluated.
\end{itemize}
Once the memory is updated with the new information, the monitor evaluates the rules and scans for a verdict.
It attempts to get a final verdict in the rules that span the timestamp it is monitoring up to the current timestamp: $\exists t_{v} \in [t_{id}, t], \exists v \in \verdictb: v = \verdictAt(\sys, \mem, t_v)$.
If such a verdict is found, it sends $\msgverdict(id, t_\mathrm{mon}, v)$ to all monitors in $\chorref$, and then considers one of the two following cases:
\begin{itemize}
	\item If it does not respawn then it terminates. If it is the root node $(\chorref = \emptyset)$ then it reports the verdict and terminates.
	\item If it does respawn, then it increments $t_\mathrm{mon}$ by one to monitor for the next timestamp, and reassigns the representation with the initial state at $t_\mathrm{mon}$, thus: $\sys := [t_\mathrm{mon} \mapsto q_0 \mapsto \vt]$, the $\chorkill$ set is cleared, and it is also possible to discard all atoms $\tuple{t_a, ap}$ from the memory that have $t_a \leq t_\mathrm{mon}$, as they would no longer be needed.
\end{itemize}

\begin{algorithm}[!tp]
\caption{Choreography}
\label{alg:choreography-monitor}

\begin{algorithmic}[1]
\Procedure{ChorMon}{$t, o$}
	\State $\mem \gets \mem \memadd \cons(o,t)$
	\While{Message $\msgkill(id_{\mathrm{from}})$ is received}
		\State $\chorkill \gets \chorkill \cup \setof{id_{\mathrm{from}}}$
		\If{$\chorkill = \chorref$} \Comment{Kill}
			\State $\forall mon \in \chorcoref : \mbox{ send } \msgkill(id)$
			\State Terminate
		\EndIf
	\EndWhile
	\While{Message $\msgverdict(id_{\mathrm{from}}, t_v, v)$ is received} \Comment{Update Verdicts}
		\State $\mem \gets \mem \memadd [\tuple{t_v, id_{\mathrm{from}}} \mapsto v]$
	\EndWhile
	\State $\sys \gets \smove(\sys, t-1, t)$
	\ForAll{$t_{v} \in [t_{id},  t]$} \Comment{Check Verdict}
		\State Rewrite the rules at $\sys(t)$ and simplify
		\State {$v = \verdictAt(\sys, \mem, t_{v})$}
		\If{$v \in \verdictb$}
			\If{$\chorref = \emptyset$} \Comment{Top-Level Monitor}
				\State Report verdict $v$ and terminate.
			\Else
				\State $\forall mon \in \chorref \setminus \chorkill : \mbox{ send } \msgverdict(id, t_{id}, v)$
				\If{$respawn_{id}$} \Comment{Respawn}
					\State $\sys \gets [t_{id} \mapsto q_0 \mapsto true]$
					\State $t_{id} \gets t_{id} + 1$
					\State $\chorkill \gets \emptyset$
				\Else
					\State $\forall mon \in \chorcoref : \mbox{ send } \msgkill(id)$
					\State Terminate
				\EndIf
			\EndIf
		\EndIf
	\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> alg-migration.tex <==
\subsection{Migration}
The migration algorithm initially consists in migrating the monitor from one or more component to other  components to fill in missing observations.
Since in our $\MemRep{}$ encoding we guarantee that two monitors receiving the same information are in the same state, it amounts to rewriting the $\MemRep{}$ and migrating it across components. 

In our setup, the migration algorithm will assign a monitor per component.
These monitors are strongly connected; each monitor is connected to all other monitors.
The monitors are either active or inactive.
Active monitors are monitors that seek to find a verdict while inactive monitors are idle, waiting for other monitors to send them their \MemRep{}.
Both active and inactive monitors store the observations they receive in their memory.
However, only active monitors will update the expressions in their $\MemRep{}$.
After expression are updated, active monitors will determine which other monitors should be sent the $\MemRep{}$ to continue monitoring.
To determine the next monitor, the function $\migrchc : \timestamp \times Q \rightarrow \comps$ is used on an $\MemRep{}$ to return the next component.
The $\migrchc$ function finds the atom $\tuple{t_{min}, \vars{ap}}$ with the smallest timestamp in each expression in $\sys$, and checks which component can observe $\vars{ap}$.
To determine which monitors are initially active, each monitor does one move then checks whether or not its component is the outcome of $\migrchc$.

\begin{algorithm}
 \caption{Migration}
 \label{alg:migration}

\begin{algorithmic}[1]
\Procedure{Migration}{$t, o$}
	\State $\mem \gets \mem \memadd \cons(o, \fts_t)$
	\While{Received $\sys'$}
		\If{$isActive$}
			\State $\sys \gets \sys \sysadd \sys'$\Comment{Merge information}
		\Else
			\State $\sys \gets \sys'$ 
			\State $isActive \gets \vt$
		\EndIf
	\EndWhile
	\If{$isActive$}
		\State $\sys \gets \smove(\sys, t-1, t)$
		\State Rewrite each rule in $\sys$ and simplify it
		\ForAll{$t_v \in dom(\sys)$} \Comment{Go through all $\MemRep{}$ timestamps}
			\State $v \gets \verdictAt(\sys, \mem, t_v)$
			\If{$v \in \verdictb$}
					\State Report $v$ and terminate
			\EndIf
		\EndFor
		\State $c_k \gets \migrchc(\sys)$ \Comment{Migrate}
		\If{$c_k \neq c$}
			\State $isActive \gets \vf$
			\State Send $\sys$ to $\MONID_k$
		\EndIf
	\EndIf	
\EndProcedure
\end{algorithmic}

\end{algorithm}

\ralg{alg:migration} shows the migration algorithm adapted for $\MemRep{}$.
At each timestamp $t$, each monitor updates their memory with the new set of observations.
The monitor then checks whether or not it received an $\MemRep{}$ from other monitors.
If it received an $\MemRep{}$ $\sys'$, and is monitoring, it merges it with its \MemRep{}, otherwise it replaces it with what it receives.
If the monitor is monitoring, then it does one move, and evaluates the rules based on its memory.
Then checks for all $t_v \in dom(\sys)$ whether or not it can find a verdict.
If a verdict is found, then it is reported, otherwise, it determines whether or not it should send $\sys$ to another monitor.


==> alg-orchestration.tex <==
\subsection{Orchestration}
The orchestration algorithm consists in setting up a main monitor which will be in charge of monitoring the entire specification.
However since that monitor cannot have access to all observations on all components, orchestration introduces one monitor per component to forward the observations to the main monitor.



\paragraph{Centralized specification.}
In the case of a centralized specification, we create a main monitor $\MONID_0$, and place it on component $c_0$.
The monitor $\MONID_0$ will be performing the monitoring by receiving all observations from other components.
To send observations we create $|\comps| - 1$ forwarding monitors on the rest of the components.
The forwarding monitors are then labelled $F = \setof{\MONID_k \mid  k \in [1, |\comps|]}$.
The network graph is then: $\tuple{\setof{\MONID_0} \cup F, \setof{\tuple{m, \MONID_0} \mid m \in F}}$
%
~
We show how monitoring is done in $\ralg{alg:orch-c}$ with the two procedures \vars{OrchSub} and \vars{OrchMain} that describe the forwarding and main monitor respectively.
The configuration of the main monitor consists of a triple $\tuple{t_{\mathrm{kn}}, \mem, \sys^0}$ with $\sys^0$ initialized to $\sys^0 = [0 \mapsto q_0 \mapsto \vt]$.
The $t_\mathrm{kn}$ is used to store the timestamp of the  last found state and it is initialized to 0.
Each forwarding monitor has knowledge of the component it is bound to.

\begin{algorithm}
 \caption{Centralized Orchestration}
 \label{alg:orch-c}
\begin{algorithmic}[1]

\Procedure{OrchSub}{$t, o$}
	\State Send  $\cons(o, \fts_t)$ to $\MONID_0$
\EndProcedure

\Procedure{OrchMain}{$t$}
	\While{Receive $\mem'$ from an $OrchSub$} \Comment{Merge Memory}
		\State $\mem \gets \mem \memadd \mem'$
	\EndWhile
	\State $\sys \gets \smove(\sys, t-1, t)$
	\State $t_f \gets \func{scanState}(\sys, \mem, t_\mathrm{kn} + 1, t)$
	\If{$t_f > t_\mathrm{kn}$}
		\State $t_\mathrm{kn} \gets t_f$
		\State $v \gets \verdictAt(\sys, \mem, t_\mathrm{kn})$
		\If{$v \in \verdictb$}
			\State Report $v$ and terminate
		\EndIf
	\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

The main monitor $\MONID_0$ receives memories from all forwarding monitors and combines them in its memory ($\mem \gets \mem \memadd \mem'$).
Then makes a move $\sys \gets \smove(\sys, t-1, t)$ then attempts to find the new state of the automaton execution given the new information it received.
If a new state is found, it checks if its a final verdict, and if it is, it reports it.
The forwarding monitor simply forwards the memory creating from the observations ($\cons(o, \fts_t)$).
We note that by using $\MemRep{}$ to encode the execution, it is possible to see that the Orchestration algorithm tolerates out-of-order messages, so long as they are eventually delivered.

\paragraph{Decentralized specification.}
Another approach to handle orchestration is to generate an equivalent decentralized specification (as in \rsec{sec:dmon}).
To do so, we consider each atomic propositions $ap \in \AP$ in the main formula to be monitored at the component where it can be observed with the simple monitor that checks for either $ap$ or $\neg ap$.
All of these monitors send their verdict to a central monitor that handles monitoring the global formula.
The central monitor can be attached to any component as it is not labeled with atomic propositions, but with the ids of the monitors monitoring the atomic propositions.

\getfig{alg-orch}{Monitoring $\mathrm{F}(a_0 \lor b_0)$ with orchestration}{fig:specorch}

\begin{example}[Orchestration] \label{ex:alg-orchestration}
We adapt \rex{ex:dmon:aut} to monitor $F(a_0 \lor b_0)$ using orchestration and show the specifications in \rfigb{fig:specorch}.
In this case, we use two monitors ($\MONID_1, \MONID_2$) to monitor $a_0$ and $b_0$.
The monitor $\MONID_1$ (resp. $\MONID_2$) is attached to component $A$ (resp. $B$).
The monitor $\MONID_0$ represents the main monitor and can be placed on either $A$ or $B$ as its specification is not labeled with atomic propositions.
\end{example}


 


==> algs.tex <==
\section{Decentralized Monitoring Algorithms} \label{sec:algs}
In this section, we start by introducing a general decentralized monitoring algorithm, then adapt the existing three algorithms: Orchestration, Migration and Choreography\cite{DecentMon} to the model presented, and the automata representation discussed in the previous section.
We note that these algorithms operate over a global clock, therefore the sequence of steps can be directly mapped to the timestamp.
Additionally, we choose an appropriate encoding of $\atoms$ to consist of a timestamp and the atomic proposition ($\atoms = \timestamp \times \AP$).
These algorithms are originally presented using an LTL specification instead of automata, however, it is possible to obtain an equivalent Moore automaton as described in \cite{LTL3Tools}.

~

A decentralized monitoring algorithm takes as input a decentralized trace and specification and outputs a verdict.
To determine the verdict, a decentralized monitoring algorithm consists of two steps: setting up the monitoring network, and monitoring.
In the first step, the algorithm initializes the monitors, defines the way they are connected to each other, and attaches them to the components that require monitoring.
We represent the connections between the various monitors using a directed graph $\tuple{\mons, E}$ that represents the monitor network where $\mons$ represents the set of monitors as described in \rsec{sec:dmon}, and $E = 2^\mons \times \mons$ describing the sender-receiver relationship between monitors.
For example, the network $\tuple{\setof{\MONID_0, \MONID_1}, \setof{\tuple{\MONID_1, \MONID_0}}}$ describes a network consisting of two monitors $\MONID_0$ and $\MONID_1$ where $\MONID_1$ sends information to $\MONID_0$.
In the second step, a decentralized monitoring algorithm proceeds with the monitoring, wherein each monitor processes observations and communicates with other monitors.

~

\begin{algorithm}
 \caption{Scan State}
 \label{alg:scan}
\begin{algorithmic}[1]
\Function{scanState}{$\sys, \mem, t_s, t_e$}
	\State $t_{kn} \gets 0$
	\ForAll{$t \in [t_s, t_e]$}
		\State $q \gets \sreach(\sys, \mem,  t)$
		\If{$q \neq \fundef$}
			\State $t_{kn} \gets t$
		\EndIf
	\EndFor
	\State\Return $t_{kn}$
\EndFunction
\end{algorithmic}
\end{algorithm}

Before we adapt existing algorithms to use $\MemRep{}$, we first present a common function $\vars{scanState}$ in \ralg{alg:scan}.
The $\vars{scanState}$ function returns the timestamp of the last found state within a given timestamp range $[t_s, t_e]$.


\input{alg-orchestration}
\input{alg-migration}
\input{alg-choreography}


==> arch0.tex <==
\section{Architecture} \label{sec:arch}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
A key advantage of decentralized specifications is the ability to associate monitors to components.
This allows us to map the monitor network to the actual system architecture constraints.

The monitor network is a graph $N = \tuple{V, E}$ with two cost functions $\mathrm{C_p}$ and $\mathrm{C_c}$ that label the nodes and edges, respectively.
\begin{itemize}
	\item $V$ is the set of monitors;
	\item $E$ is the edges representing communication between monitors;
	\item $\mathrm{C_p}$ is the processing requirement of a monitor (computation);
	\item $\mathrm{C_c}$ is the cost of the communication between any two monitors (size/number of messages).
\end{itemize}

The system is represented as another graph $S = \tuple{V',E'}$ with two cost functions $\mathrm{A_p}$ and $\mathrm{A_c}$ that label the nodes and edges, respectively.
\begin{itemize}
	\item $V'$ is the set of components;
	\item $E'$ is a set of communication channels between components;
	\item $\mathrm{A_p}$ represents the processing power of a component (Available Processing);
	\item $\mathrm{A_c}$ represents the communication channel bandwidth (Available Communication).
\end{itemize}

The following problems are then needed to solve.
We have a simplified case where $|V'| = |V|$.

\paragraph{Compatibility.}

Informally: Can the monitor network (typically synthesized by the spec) be deployed on the system?

Formally: Is there a mapping $R : V \rightarrow V'$ such that:
\[
	\forall v_1, v_2 \in V, \mathrm{reach}(v_1, v_2) \mbox{ iff } \mathrm{reach}(R(v_1), R(v_2))
\]

where $\mathrm{reach}(v_1, v_2)$ indicates that $v_2$ is reachable from $v_1$.


Hint: This problem is a relaxed form of graph homomorphism modulo reachability (homomorphism preserving reachability).

\paragraph{Compatibility Synthesis}

Given a centralized specification that needs to be decentralized over $n$ components such that we have one monitor per component ($|\comps| = |V| = n$).
Let $\tuple{V',E'}$ be the system graph.
Find a decentralized specification $\aut_0 \hdots \aut_n$ with a monitor network $\tuple{V,E}$ such that:
\begin{enumerate}
		\item $\tuple{V,E}$ is compatible with $\tuple{V',E'}$
		\item $\forall v_1, v_2 \in V \quad  \aut_{v_2} \in \mondep(\aut_{v_1}) \implies \tuple{v_2, v_1} \in E $
		\item (Complete) $\forall v \in V \quad \monitorable(v)$
\end{enumerate}


\paragraph{Optimization.}

Informally: What is the best assignment of monitors to components that minimizes both computation overhead and communication overhead.

\todo[inline]{This is posited as mapping edges as well, however needs to be changed to flow}
Formally: Find mapping $R : V \rightarrow V'$ that minimizes the double sum:
\[
	\Sigma_{v \in V} [ (\mathrm{C_p}(v) - \mathrm{A_p}(R(v))) +  \mathrm{C_c}(v) - \mathrm{A_c}(R(v))) ]
\]
with the constaint:
\[
	\forall v \in V, \mathrm{C_c(v)} \leq A_c(R(v))
\]


==> decent.tex <==
\section{Common Notions} \label{sec:common}
%
We begin by introducing the \vars{dict} data structure used to build more complex data structures in \rsec{sec:common:dict}.
Then, we introduce the basic concepts for decentralized monitoring in \rsec{sec:common:mon}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The \vars{dict} Data Structure}
\label{sec:common:dict}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In monitoring decentralized systems, monitors typically have a state, and attempt to merge other monitor states with theirs to maintain a consistent view of the running system, that is, at no point in the execution, should two monitors receive updates that conflict with one another.
%
We would like in addition, that any two monitors receiving the same information be in equivalent states.
%
Therefore, we are interested in designing data structures that can replicate their state under strong eventual consistency (SEC)~\cite{CRDT}, they are known as  state-based convergent replicated data-types (CvRDTs).
%
We  use a dictionary data structure \vars{dict} as our basic building block that maps a key to a value.
%
\vars{dict} supports two operations: $\vars{query}$ and $\vars{merge}$.
%
The $\vars{merge}$ operation is the only operation that modifies \vars{dict}.
%
The modifications never remove entries, the state of \vars{dict} is then monotonically increasing.
%
By ensuring that $\vars{merge}$ is idempotent, commutative, and associative we fulfill the necessary conditions for our data structure to be a CvRDT.
%
\begin{proposition}
\label{prop:common:dict}
Data structure \vars{dict} with operations $\vars{query}$ and $\vars{merge}$ is a CvRDT.
\end{proposition}
%
We model \vars{dict} as a partial function $\func{f}$.
The keys are the domain of $\func{f}$, i.e., $\fdom(\func{f})$ and values are mapped to each entry of the domain.
%
The $\vars{query}$ operation checks if a key $k \in \fdom(\func{f})$ and returns $\func{f}(k)$.
If $k \not\in \fdom(\func{f})$, then it is $\fundef$.
The $\vars{merge}$ operation of a \vars{dict} $f$ with another \vars{dict} $g$, is modeled as function composition.
%
Two partial functions $\func{f}$ and  $\func{g}$ are composed using operator $\dagger_{\mathit{op}}$ where $\mathit{op} : (\fdom(f) \times \fdom(g)) \rightarrow (\fcodom(f) \cup \fcodom(g))$ is a binary function.
%
\begin{align*}
	\func{f} \dagger_{\mathit{op}} \func{g}(\xv) 	 &: \fdom(\func{f}) \cup \fdom(\func{g}) \rightarrow \fcodom(\func{f}) \cup \fcodom(\func{g})\\
							 &= \funcparts{
		op(\func{f}(\xv), \func{g}(\xv))	 	 & \pif \xv \in 		\fdom(\func{f}) \cap \fdom(\func{g})\\
		\func{g}(\xv)				 & \pif \xv \in \fdom(\func{g}) \setminus \fdom(\func{f})\\
		\func{f}(\xv)				 & \pif \xv \in		\fdom(\func{f}) \setminus \fdom(\func{g})\\
		\fundef				 & \pelse
}
\end{align*}
%
On sets of functions, $\dagger_{\mathit{op}}$ applies pairwise: $\biguplus^{\mathit{op}}\setof{\func{f_1}, \hdots \func{f_n}} =$ $((\func{f_1} \dagger_{op} \func{f_2}) \hdots \func{f_n})$
%
The following two operators are used in the rest of the paper: $\memadd$ and $\sysadd$.
%
We define both of these operators to be commutative, idempotent, and associative to ensure SEC.
\begin{align*}%
  \memadd(\xv,\xv') = \funcparts{
  \xv' & \pif \xv \prec \xv'\\
  \xv  & \xelse \\
} & \quad
\sysadd(\xv, \xv') = \xv \lor \xv'
\end{align*}
%
Operator $\memadd$ acts as a replace function with the addition of a total order ($\prec$) between the elements, so that it always chooses the highest element to guarantee idempotence, while $\sysadd$ is simply the logical \emph{or} operator.
%
Respectively, we denote the pairwise set operators as $\biguplus^{2}$ and $\biguplus^{\lor}$.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Basic Monitoring Concepts} \label{sec:common:mon}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
We recall the basic building blocks of monitoring.
%
We consider the set of verdicts $\verdict = \setof{\vt, \vf, \vna}$ to denote the verdicts true, false, not reached (or inconclusive) respectively.
%
A verdict from $\verdictb = \setof{\vt, \vf}$ is a \emph{final} verdict.
%
Given a set of atomic propositions $\AP$, we define an encoding of the atomic propositions as $\atoms$, this encoding is left to the monitoring algorithm to specify.
%
$\expr_\atoms$ (resp. $\expr_\AP$) denotes the set of boolean expressions over $\atoms$ (resp. $\AP$).
%
When omitted, $\expr$ refers to $\expr_\atoms$.
%
An encoder is a function $\senc : \expr_\AP \rightarrow \expr_\atoms$ that encodes the atomic propositions into atoms.
%
In this paper, we use two encoders: $\fid$ which is the identity function (it does not modify the atomic proposition), and $\fts_t$ which adds a timestamp $t$ to each atomic proposition.
%
A decentralized monitoring algorithm requires retaining, retrieving and communicating observations.
%
\begin{definition}[Event]
\label{def:common:event}
	An observation is a pair in $\AP \times \verdictb$ indicating whether or not a proposition has been observed. An event is a set of observations in $2^{\AP \times \verdictb}$.
\end{definition}
%
\begin{example}[Event]\label{ex:common:event}
 The event $\setof{\tuple{a, \vt}, \tuple{b, \vf}}$ over $\AP = \setof{a,b}$ indicates that the proposition $a$ has been observed to be true, while $b$ has been observed to be false.
\end{example}
%
\begin{definition}[Memory]
\label{def:common:mem}
A memory is a \vars{dict}, and is modeled as a partial function $\mem : \atoms \rightarrow \verdict$ that associates an atom to a verdict.
The set of all memories is defined as $\Mem$.
\end{definition}
%
Events are commonly stored in a monitor memory with some encoding (e.g.,  adding a timestamp).
%
An event can be converted to a memory by encoding the atomic propositions to atoms, and associating their truth value: $\cons: 2^{\AP \times \verdictb} \times (\expr_\AP \rightarrow \expr_\atoms) \rightarrow \Mem$.
%
\begin{example}[Memory]\label{ex:common:mem}
Let $e$ $=$ $\setof{\tuple{a, \vt}, \tuple{b, \vf}}$ be an event at $t = 1$, the resulting memories using our encoders are:\\
$\begin{array}{ll}
	\cons(e, \fid) &= [a \mapsto \vt, b \mapsto \vf],\\
	\cons(e, \fts_1) &= [\tuple{1, a} \mapsto \vt, \tuple{1, b} \mapsto \vf].
\end{array}$
\end{example}
%
If we impose that $\atoms$ be a totally ordered set, then two memories $\mem_1$ and $\mem_2$ can be merged by applying operator $\memadd$.
%
The total ordering is needed for the operator $\memadd$.
%
This ensures that the operation is idempotent, associative and commutative.
%
Monitors that exchange their memories  and merge them  have a consistent snapshot of the memory, regardless of the ordering.
%
Since memory is a \vars{dict} and $\memadd$ is idempotent, associative, and commutative, it follows from \rprop{prop:common:dict} that it is a CvRDT.
%
\begin{corollary}\label{prop:mem-crdt}
A memory with operation $\memadd$ is a CvRDT.
\end{corollary}
%
In this paper, we perform monitoring by manipulating expressions in $\expr$.
%
The first operation we provide is $\rw$, which rewrites the expression to attempt to eliminate $\atoms$.
%
\begin{definition}[Rewriting]
\label{def:common:rw}
An expression $\vars{expr}$ is rewritten with a memory $\mem$ using $\rw(\vars{expr},\mem)$ defined as follows:
\begin{align*}
	\rw & : \expr \times \Mem \rightarrow \expr\\
	\rw(\vars{expr}, \mem) &= \texttt{ match $\vars{expr}$ with }\\
				 & \begin{array}{ll}
				\mid a \in \atoms  & \rightarrow \funcparts {
						\mem(a)		& \pif a \in dom(\mem)\\
						a			& \pelse
				}\\
				\mid \neg e		   & \rightarrow \neg \rw(e, \mem)\\
				\mid e_1 \land e_2 & \rightarrow \rw(e_1,\mem) \land \rw(e_2, \mem)\\
				\mid e_1 \lor e_2 & \rightarrow \rw(e_1,\mem) \lor \rw(e_2, \mem)
\end{array}
\end{align*}
\end{definition}
%
Using information from a memory $\mem$, the expression is rewritten by replacing atoms with a final verdict (a truth value in $\verdictb$) in $\mem$ when possible.
%
Atoms that are not associated with a final verdict are kept in the expression.
%
The operation $\rw$ yields a smaller formula to work with and repeatedly evaluate.
%
\begin{example}[Rewriting]
\label{ex:common:rw}
We consider $\mem = [a \mapsto \vt, b \mapsto \vf];$ and $e = (a \lor b) \land c$.
%
We have $\mem(a) = \vt$, $\mem(b) = \vf$, $\mem(c) = \vna$.
%
Since $c$ is associated with $\vna \not\in \verdictb$ then it will not be replaced.
%
The resulting expression is $\rw(e,\mem) = (\vt \lor \vf)\land c$.
\end{example}
%
We eliminate additional atoms using boolean logic.
%
We denote by $\fsimp(\vars{expr})$ the simplification of formula $\vars{expr}$~\footnote{This is also known as The Minimum Equivalent Expression problem~\cite{CircuitMin}.}.
%
\begin{example}[Simplification] \label{ex:common:simplify}
Consider $\mem = [a \mapsto \vt]$ and  $e = (a \land b) \lor (a \land \neg b)$.
%
We have $e' = \rw(e, \mem) = (b \lor \neg b)$.
%
Atoms can be eliminated with $\fsimp(e')$.
%
We finally get $\vt$.
\end{example}
%
We combine both rewriting and simplification in the $\seval$ function which determines a verdict from an expression $\vars{expr}$.
%
\begin{definition}[Evaluating an expression]
\label{def:common:eval}
The evaluation of an boolean expression $\vars{expr} \in \expr$ using a memory $\mem$ yields a verdict. $\seval: \expr \times \Mem \rightarrow \verdict$:
%
\begin{align*}
	\seval (\vars{expr}, \mem) &= \funcparts{
      \vt & \pif e' \Leftrightarrow \vt\\
      \vf & \pif e' \Leftrightarrow \vf\\
      \vna& \pelse
   }\\
  \mbox{\text{with }} & e' = \fsimp(\rw(\vars{expr}, \mem))
\end{align*}
\end{definition}
%
Function $\seval$ returns the $\vt$ (resp. $\vf$) verdict if the simplification after rewriting is (boolean) equivalent to  $\vt$ (resp. $\vf$), otherwise it returns the verdict $\vna$.
%
\begin{example}[Evaluating expressions]\label{ex:common:eval}
Consider $\mem = [a \mapsto \vt, b \mapsto \vf]$ and $e = (a \lor b) \land c$.
ù
We have $\fsimp(\rw(e, \mem)) = \fsimp((\vt \lor \vf) \land c) =  c$, and $\seval(e,\mem) = \vna$ which depends on $c$: we cannot emit a final verdict before observing $c$.
\end{example}
%
A decentralized system is as set of components $\comps$, we associate a sequence of events to each component using a decentralized trace function.
%
\begin{definition}[Decentralized trace]
\label{def:common:dtrace}
A decentralized trace is a function $\trace : \timestamp \times \comps \rightarrow 2^{\AP \times \verdictb}$.
\end{definition}
%
Function $\trace$ assigns an event to a component for a given timestamp.
%
We additionally define function $\clookup : \AP \rightarrow \comps$ to associate an observation to a component\footnote{We assume that (1) no two components can observe the same atomic propositions, and (2) a component has at least one observation at all times (a component with no observations to monitor, can be simply considered excluded from the system under monitoring).}.\\
%
$\clookup(ap) = c \mbox { s.t. } \exists t \in \timestamp, \exists v \in \verdictb : \tuple{ap, v} \in \trace(t, c)$.

We consider timestamp 0 to be associated with the initial state, therefore our traces start at 1.
%
Thus, a finite trace  of length $n$ is a function $\trace$ with a domain $[1, n]$.
%
An empty trace has length 0 and is denoted by $\emptyset$.
%
While $\trace$ gives us a view of what components can locally see, we reconstruct the global trace to reason about all observations.
%
\begin{definition}[Reconstructing a global trace]
\label{def:common:gtrace}
Given a decentralized trace $\trace$ of length $n$, the global trace $\rho(\trace) = e_1 \cdot \hdots \cdot e_{n}$ is s.t. $\forall i \in [1, n] : e_i = \bigcup_{c \in \comps} \trace(i, c)$.
\end{definition}
%
For each timestamp $i \in [1, n]$ we take all observations of all components and union them to get a global event.
%
Consequently, an empty trace yields an empty global trace, $\rho(\emptyset) = \emptyset$.
%


==> paper.tex <==
\begin{document}
\input{title}
\input{abstract}
\input{intro}
\input{rw}
\input{common}
\input{cmonitoring}
\input{dmonitoring}
\input{algs}
\input{analysis}
\input{tool}
\input{experiment}
\input{conclusion}

\appendix
\input{appendix}

%%__References__%
\bibliographystyle{splncs03}
\bibliography{biblio}
%

\end{document}


==> temp.tex <==
\section{Common Notions}
\subsection{Override $\memadd$}
\begin{align*}
	f \memadd f'(x) &: dom(f) \cup dom(f') \rightarrow codom(f) \cup codom(f') \\
		 &= \funcparts{
			f'(x) & \mbox{if } x \in dom(f')\\
			f(x)  & \mbox{otherwise}	
	}
\end{align*}



\subsection{Atoms}
A distributed monitoring algorithm defines a set of atomic propositions $\atoms$.
$\expr$ denotes the set of boolean expressions over $\atoms$.

\subsection{Memory}
A memory $\mem$ is a partial function that associates an atom in $\atoms$ to a verdict:
\begin{align*}
	\mem(a) : X \subseteq(\atoms) \rightarrow \verdict\\
\end{align*}
\\
Accessing an element in a memory is defined as:
\begin{align*}
	\mem[a] = \twopartdef{\mem(a)}{a \in dom(\mem)}{?}
\end{align*}

\subsection{Evaluating Expressions}
\begin{align*}
	\eval(exp, mem) &: \expr \times \mem \rightarrow \verdict\\
					&= \texttt{match $exp$ with:}\\
					& \quad\quad \begin{array}{l l}
			|\> a \in \atoms & \rightarrow mem[a] \\
			|\> \neg \phi & \rightarrow \neg \eval(\phi, mem) \\
			|\> \phi \land \phi' & \rightarrow eval(\phi, mem) \land eval(\phi', mem) \\
			|\> \phi \lor \phi' & \rightarrow eval(\phi, mem) \lor eval(\phi', mem) \\
			|\> \epsilon  & \rightarrow ? \\
	\end{array}
\end{align*}

\subsection{Specification}
The input of a distributed monitoring algorithm is an LTL specification $\varphi$. However internally $\varphi$ is converted to an automaton $\aut = \tuple{Q, \expr, \delta, \verdictf, q_0}$ where:
\begin{itemize}
	\item $\delta : Q \times \expr \rightarrow Q$
	\item $\verdictf : Q \times \verdict$
\end{itemize}

\noindent
Determining an automata state is done by using the partial function $\sys$ that associates a timestamp and a state to an expression:
$\sys : \timestamp \times Q \rightarrow \expr$

\noindent
Given a memory $\mem$, a verdict at timestamp $t$ is determined by
\[
	verdictAt(\aut, \sys, \mem, t) = \twopartdef
					{\verdictf(q)}{\exists q : eval(\sys(t,q), \mem) = true}
					{?} 
\] 

\begin{align*}
	\sys \overload \sys'(x) &: dom(\sys) \cup dom(\sys') \rightarrow codom(\sys) \cup codom(\sys')\\
						 &= \funcparts{
							\sys(x) \lor \sys'(x) & \mbox{if } x \in dom(\sys) \> \land x \in dom(\sys')\\
							\sys'(x) 			  & \mbox{if } x \not\in dom(\sys') \land x\in dom(\sys')\\
							\sys(x)				  & \mbox{otherwise}
						}
\end{align*}

\begin{align*}
	move(A = \tuple{Q, expr, \delta, verdict, q_0}, I, t, transform) :\\
		\aut \times \sys \times \timestamp \times (\expr \times \timestamp \rightarrow \expr) \rightarrow \sys
\end{align*}
\begin{align*}
		\quad \forall q \in I(t-1), expr = I(t-1, q) \\
			\forall q' : \delta(q, expr') = q' \\
				I := I \overload [t \mapsto q' \mapsto expr \land transform(expr', t) ]
\end{align*}


\section{Orchestration}
$\atoms = ap \cup \tuple{\timestamp \times ap}$

\begin{align*}
	convert(exp, t) : & \expr \times \timestamp \rightarrow \expr\\
					= & \texttt{ match exp with}\\
					  & \begin{array}{ll}
					| \> a \in ap  & \rightarrow \, \tuple{t, ap} \\
					| \> \neg \phi & \rightarrow \, \neg convert(\phi, t)\\
					| \> \phi \land \phi' & \rightarrow \, convert(\phi, t) \land convert(\phi', t) \\
					| \> \phi \lor \phi' & \rightarrow \, convert(\phi, t) \lor convert(\phi', t) \\
	\end{array}
\end{align*}
~

\noindent
Main Monitor:
\begin{enumerate}
	\item Given $\phi$ construct $\aut$, initialize:\\
			$t_{last} = 0$, $\mem := [\quad]$, $\sys := [0 \mapsto q_0 \mapsto true]$.
	\item When receiving $\mem'$ from a submonitor:
		\begin{enumerate}
			\item $\mem = \mem \memadd \mem'$
			\item Let $t_{max}$ : $\exists \tuple{t_{max},a} \in dom(\mem), \not\exists \tuple{t',a'} \in dom(\mem) \texttt{ s.t } t' > t_{max}$
			\item if($t_{max} > t_{last}$):
				\begin{enumerate}
					\item for $t = [t_{last} + 1 \hdots t_{max}]$:  $move(\aut, \sys, t, convert)$
					\item $t_{last} := t_{max}$
				\end{enumerate}
			\item for $t = [1 \hdots t_{last}]$:\\
			if ($verdictAt(\aut, \sys, \mem, t) \neq ?)$ report and terminate
		\end{enumerate}
\end{enumerate}

Submonitor:
\begin{enumerate}
	\item On observing $a \in ap$ to be $v \in \verdict$ at timestamp $t$
	\item Send $[\tuple{t,a} \mapsto v]$ to main monitor
\end{enumerate}


\section{Migration}
Given an original specification all monitors construct the automata $\aut$

On a timestamp $t$
\begin{itemize}
	\item On an observation $a \in ap$ to be $v$: $\mem := \mem \memadd [\tuple{t, ap} \mapsto v]$.
	\item If not monitoring formula and received formula $\sys'$:
	\begin{enumerate}
		\item $\sys := \sys'$
		\item Jump to monitoring
	\end{enumerate}
	\item (Monitoring) If monitoring formula:
	\begin{enumerate}
		\item If received formula $\sys'$, $\sys := \sys \memadd \sys'$
		\item $move(\aut, \sys, t, convert)$
		\item for $t' = [1 \hdots t]$\\
			if ($verdictAt(\aut, \sys, \mem, t) \neq ?)$ report and terminate
		\item Determine if need to send $\sys$ and send if needed
	\end{enumerate}
\end{itemize}



\newpage

~


\newpage

~


\newpage


\section{Orchestration}
\begin{enumerate}
	\item Construct $\aut = \tuple{Q,  \Sigma, \delta , verdict, q_0} $from LTL spec where:
	\begin{itemize}
		\item $\delta : Q \times \Sigma \rightarrow Q$
		\item $L : Q \rightarrow \verdict $ 
	\end{itemize}
	\item Set $q_c = q_0$
	\item Loop for $t = 1 \hdots n$ :
	\begin{enumerate}
		\item Wait to receive all observations to form the event $\sigma$ 
		\item Move to $\delta(q_c, \sigma) = q'$
		\item Set $q_c = q'$
		\item Emit verdict $\tuple{t, verdict(q_c)}$ 
	\end{enumerate}
	
\end{enumerate}


\section{Migration}

\subsection{Structure of the Monitor}
A monitor is a tuple $\tuple{Q, \Sigma, \delta, verdict, q_0, \mem, \sys }$ where:
\begin{itemize}
	\item $Q$ is the set of states;
	\item $\Sigma = 2^{AP}$ is the alphabet of events;
	\item $delta : Q \times \Sigma \rightarrow Q$ the complete transition function;
	\item $verdict: Q \rightarrow \verdict$ the verdict function;
	\item $q_0$ the initial state;
	\item $\sys : \timestamp \times Q \rightarrow Expr(\timestamp \times AP)$ denotes a set of inferences at timestamp $t$.
		\begin{itemize}
			\item $\sys(0, q_0) = true$
		\end{itemize}
\end{itemize}

\subsection{Operations}

\subsubsection*{Evaluating Timed Observations}
%\[
%get(\tuple{t, \sigma}, \mem) =  \twopartdef{\tuple{t, \mem(t, \sigma)}} {\mem(t, \sigma) \neq ?}
%				{\tuple{t, \sigma}}
%\]

$eval(expr, \mem) = $ match $expr$ with:
\[
\begin{array}{|l l}
	 true \land expr & \rightarrow expr\\
	true \lor   expr & \rightarrow true\\
	false \land expr & \rightarrow false\\
	false \lor   expr & \rightarrow expr\\
	? \land expr & \rightarrow ?\\
	? \lor   expr & \rightarrow expr\\
	\tuple{n, true} \quad op \quad expr & \rightarrow true \quad op \quad expr\\
	\tuple{n, false} \quad op \quad expr & \rightarrow false \quad op \quad expr\\
	\tuple{n, \sigma}  \quad op  \quad expr & \rightarrow \mem(n, \sigma) \quad op \quad  expr\\
\end{array}
\]


\subsubsection*{Verdict at $t$}
\[
resolve(\sys, t,\mem, verdict) =  \twopartdef{verdict(q)} {\exists expr = \sys(t, q) : eval(expr, \mem) = true }
				{?}
\]


\subsubsection*{Merge}

$merge(\sys, \sys', t) = \sys(t,q, expr \lor expr' / expr) \quad \forall expr = \sys(t,q), \forall expr' = \sys'(t,q)$


~


$merge(\sys, \sys', t) = 	\left\{
		\begin{array}{ll}
			expr \lor expr'  & \mbox{if } \exists q : expr = \sys(t,q) \land expr' = \sys'(t,q) \\
			expr & \mbox{if } \exists q : expr = \sys(t,q) \land \sys'(t,q) \text{ is undefined} \\
			expr' & \mbox{if } \exists q : expr' = \sys'(t,q) \land \sys(t,q) \text{ is undefined}\\
			undefined & \mbox{otherwise}
		\end{array}
	\right.$

%$merge(I_t, I'_t)$: For $\tuple{q', expr'} \in \sys_t'$:
%\begin{itemize}
%	\item If $\exists \tuple{q', expr} \in I_t$: $I_t := (I_t \setminus   \tuple{q', expr}) \cup\{ \tuple{q', expr \lor expr'}\}$
%	\item Else: $I_t := I_t \cup \tuple{q', expr'}$
%\end{itemize}


~

%$merge(I_t, I'_t)$: For $\tuple{q', expr'} \in \sys_t'$:
%\begin{itemize}
%	\item If $\exists \tuple{q', expr} \in I_t$: $I_t := (I_t \setminus   \tuple{q', expr}) \cup\{ \tuple{q', expr \lor expr'}\}$
%	\item Else: $I_t := I_t \cup \tuple{q', expr'}$
%\end{itemize}
%$merge(I, I', t)$:
%\begin{itemize}
%	\item if $\exists q' : l'(t, q') = expr'$ : I(t,q'
%	\item Else: $I_t := I_t \cup \tuple{q', expr'}$
%\end{itemize}


~

%\noindent
%$ merge(\sys, \sys')$:
%\begin{itemize}
%	\item For $k = 0 \hdots (|\sys'| - 1): merge(\sys_k, \sys_k')$ 
%\end{itemize} 

\subsubsection*{Update}
$toExpr(t, event) : \timestamp \times \Sigma \rightarrow Expr(\timestamp \times AP)$

\jump
\noindent
$toExpr(2, \overline{ab}) \rightarrow \neg\tuple{2,  a} \lor\neg\tuple{2, b}$ 

\jump
\noindent
$update(\sigma, t, Q, \delta, \mem, \sys) :$
\begin{enumerate}
	\item match $\sigma$ with: 
\[
\begin{array}{|l l}
	 \sigma & \rightarrow \mem(t, \sigma) := true\\
	\overline{\sigma}  & \rightarrow \mem(t, \sigma) := false\\
\end{array}
\]	
	\item For $\tuple{q, expr} \in \sys_{t-1}: \delta(q, \sigma') = q'$: $merge(\sys_t, \{\tuple{q', (expr \land  toExpr(\sigma'))}\})$
	\item For $\tuple{q, expr} \in \sys_t$, simplify $expr$
\end{enumerate}


\subsection{Algorithm}
For each component: 
\begin{enumerate}
	\item Construct monitor:  $\tuple{Q, \Sigma, \delta, verdict, q_0, \mem, \sys }$ from LTL spec where:

	\item Loop for $t = 1 \hdots n$ :
	\begin{enumerate}
		\item If received inferences $\sys'$ : $merge(\sys, \sys')$
		\item $checkVerdict(\sys, \mem, verdict, t)$
		\item For observation $\sigma$,  $update(\sigma, t, Q, \delta, \mem, \sys)$
		\item $checkVerdict(\sys, \mem, verdict, t)$
		\item Determine whether or not to send $\sys$ to different component
	\end{enumerate}
\end{enumerate}
\jump
 $checkVerdict(\sys, \mem, verdict, t): $ for $k = 0 \hdots t$
\begin{itemize}
	\item Let $v = resolve(\sys_k, \mem, verdict)$
	\item If  $v \neq ?$ : output $\tuple{k, v}$
\end{itemize}


\subsection{Replacement}
\[
	get(\tuple{t, \sigma}, \mem) = \twopartdef{\mem(t, \sigma)}{\mem(t, \sigma) \neq ?}
										{\tuple{t, \sigma}}
\]
$\sys'_t = replace(\sys_t, \mem) : 2^{Q \times Expr(\timestamp \times AP)} \rightarrow  2^{Q \times Expr(\timestamp \times AP)}$

For all $\tuple{q, expr} \in \sys_t$ we get $\tuple{q, map( (\lambda(x) \>  (get(x, \mem))), expr)}$

\begin{lstlisting}[language=lisp, escapechar=^]
(replace (^$\sys_t$^, ^$\mem$^)
  (map (lambda (r)
    (cons 
      (car r) 
      (map (lambda (x) (get(x, ^$\mem$^)))
        (cdr r))))
	^$\sys_t$^))
\end{lstlisting}

\newpage
\begin{landscape}

\subsection{Examples}
\begin{tabular}{|c|p{9cm}|p{9cm}|}
	\hline \textbf{Timestamp} & \textbf{A} & \textbf{B}\\
	\hline $0, \emptyset$ & $\sys_0^A = \tuple{q_0, true}$ & $\sys_0^B = \tuple{q_0, true}$\\
	\hline $1, ab$ 
		 & $\sys_1^A = \begin{array}{l}
				 \tuple{q_0, true \land [(1,a) \land (1, b)]}  \\
				 \tuple{q_1, \neg(1,a) \lor \neg (1, b)}
		   \end{array}$
		 & $\sys_1^B = \begin{array}{l}
				 \tuple{q_0, true \land [(1, a) \land (1,b)]}  \\
				 \tuple{q_1, \neg (1, a) \lor \neg(1,b)}
		   \end{array}$ \\	
	\hline $1, (Replace)$ 
		 & $\sys_1^A = \begin{array}{l}
				 \tuple{q_0, true \land [true \land (1, b)]}  \\
				 \tuple{q_1, false \lor \neg (1, b)}
		   \end{array}$
		 & $\sys_1^B = \begin{array}{l}
				 \tuple{q_0, true \land [(1, a) \land true]}  \\
				 \tuple{q_1, \neg (1, a) \lor false}
		   \end{array}$ \\
	\hline $1, (Simplify)$ 
		 & $\sys_1^A = \begin{array}{l}
				 \tuple{q_0, (1, b)}  \\
				 \tuple{q_1, \neg (1, b)}
		   \end{array}$
		 & $\sys_1^B = \begin{array}{l}
				 \tuple{q_0, (1, a)}  \\
				 \tuple{q_1, \neg (1, a)}
		   \end{array}$ \\


	\hline $2, a\overline{b}$ 
		 & $\sys_2^A = \begin{array}{l}
				 \tuple{q_0, [(1,b) \land ((2,a) \land (2,b))]}  \\
				 \tuple{q_1, [(1,b) \land (\neg (2,a) \lor \neg (2,b))] \lor [\neg(1,b) \land true]}
		   \end{array}$
		 & $\sys_2^B = \begin{array}{l}
				 \tuple{q_0, [(1,a) \land ((2,a) \land (2,b))]}  \\
				 \tuple{q_1, [(1,a) \land (\neg (2,a) \lor \neg (2,b))] \lor [\neg(1,a) \land true]}
		   \end{array}$ \\

	\hline $2, (Replace)$ 
		 & $\sys_2^A = \begin{array}{l}
				 \tuple{q_0, [(1,b) \land (true \land (2,b))]}  \\
				 \tuple{q_1, [(1,b) \land (false \lor \neg (2,b))] \lor [\neg(1,b) \land true]}
		   \end{array}$
		 & $\sys_2^B = \begin{array}{l}
				 \tuple{q_0, [(1,a) \land ((2,a) \land false)]}  \\
				 \tuple{q_1, [(1,a) \land (\neg (2,a) \lor true)] \lor [\neg(1,a) \land true]}
		   \end{array}$ \\
	\hline $2, (Simplify)$ 
		 & $\sys_2^A = \begin{array}{l}
				 \tuple{q_0, (1,b) \land (2,b)}  \\
				 \tuple{q_1, [(1,b) \land \neg (2,b)] \lor [\neg(1,b)]}
		   \end{array}$
		 & $\sys_2^B = \begin{array}{l}
				 \tuple{q_0, [false]}  \\
				 \tuple{q_1, [true]}
		   \end{array}$ \\

	\hline \multicolumn{3}{|c|}{$B \xrightarrow{\sys^B} A$}\\
	\hline (Merge) 
		& \[\begin{array}{rl}
			\sys_1^A =&\tuple{q_0, (1,b) \lor (1,a)} \\
					  &\tuple{q_1, \neg(1,b) \lor \neg(1,a)}\\
			\sys_2^A =&\tuple{q_0, [(1,b) \land (2,b)] \lor false} \\
					  &\tuple{q_1, [(1,b) \land \neg (2,b)] \lor [\neg(1,b)] \lor true}\\
		\end{array}\]
		&  \\	
	\hline (Replace) 
		& \[\begin{array}{rl}
			\sys_1^A =&\tuple{q_0, (1,b) \lor true} \\
					  &\tuple{q_1, \neg(1,b) \lor false}\\
			\sys_2^A =&\tuple{q_0, [(1,b) \land (2,b)] \lor false} \\
					  &\tuple{q_1, [(1,b) \land \neg (2,b)] \lor [\neg(1,b)] \lor true}\\
		\end{array}\]
		&  \\	
	\hline (Simplify) 
		& \[\begin{array}{rl}
			\sys_1^A =&\tuple{q_0, true} \\
					  &\tuple{q_1, \neg(1,b)}\\
			\sys_2^A =&\tuple{q_0, [(1,b) \land (2,b)]} \\
					  &\tuple{q_1, true}\\
		\end{array}\]
		&  \\	
	\hline 
\end{tabular}
\end{landscape}

\newpage
\begin{landscape}

\begin{tabular}{| c | p{9cm} | p{5cm} | p{5cm} |}
\hline	\textbf{Timestamp} & \textbf{A} & \textbf{B} & \textbf{C}\\
\hline	1, abc
	& \[\sys_1^A = \begin{array}{l}
		\tuple{q_0, (1,b) \land (1,c)}\\
		\tuple{q_1, \neg(1,b) \lor \neg(1,c)}\\
	\end{array}\]
	& \[\sys_1^B = \begin{array}{l}
		\tuple{q_0, (1,a) \land (1,c)}\\
		\tuple{q_1, \neg(1,a) \lor \neg(1,c)}\\
	\end{array}\]
	& \[\sys_1^C = \begin{array}{l}
		\tuple{q_0, (1,a) \land (1,b)}\\
		\tuple{q_1, \neg(1,a) \lor \neg(1,b)}\\
	\end{array}\]\\
\hline \multicolumn{4}{|c|}{$B \xrightarrow{\sys^B} A, C \xrightarrow{\sys^C} A$}\\
\hline Merge (A)
	& \multicolumn{3}{|l|}{$\sys_1^A = \begin{array}{l}
		\tuple{q_0, [(1,b) \land (1,c)]\lor[(1,a) \land (1,c)]\lor[(1,a) \land (1,b)]}\\
		\tuple{q_1, [\neg(1,b) \lor \neg (1,c)] \lor [\neg(1,a) \lor \neg(1,c)] \lor [\neg(1,a) \lor \neg(1,b)]}
	\end{array}$}\\
\hline Replace (A)
	& \multicolumn{3}{|l|}{$\sys_1^A = \begin{array}{l}
		\tuple{q_0, [(1,b) \land (1,c)]\lor[true \land (1,c)]\lor[true \land (1,b)]}\\
		\tuple{q_1, [\neg(1,b) \lor \neg (1,c)] \lor [false \lor \neg(1,c)] \lor [false \lor \neg(1,b)]}
	\end{array}$}\\
\hline Simplify (A)
	& \multicolumn{3}{|l|}{$\sys_1^A = \begin{array}{l}
		\tuple{q_0, (1,c)\lor(1,b)}\\
		\tuple{q_1, [\neg(1,b) \lor \neg (1,c)]}
	\end{array}$}\\
	\hline	
\end{tabular}

\end{landscape}


\section{Choreography}

\subsection{Structure of the Monitors}

A monitor  is a tuple $Mon_i = \tuple{Q^i, \Sigma, \delta^i, verdict^i, q_0^i, \mem^i, \sys^i, r^i, ref^i}$. Where:
\begin{itemize}
	\item $\delta^i : Q^i \times Expr(\timestamp \times \timestamp \times AP) \rightarrow Q^i$.
	\item $\mem^i : \timestamp \times \timestamp \rightarrow \verdict$.
	\item  $\sys^i : \timestamp \times Q^i \rightarrow Expr(\timestamp \times \timestamp):$
	\begin{itemize}
		\item $\sys^i_0 = \tuple{q_0, true}$.
	\end{itemize}
	\item $r^i$ indicates whether or not its a respawn monitor.
	\item $ref^i \subseteq 2^{Mon \setminus \{Mon_i\}}$ are the monitors that depend on the verdict of this monitor.
\end{itemize}

\subsection{Modification from Migration}

$eval(expr,\mem^i) =$ match  $expr$  with:
\[
\begin{array}{|l l}
	\tuple{t, i}  \quad op  \quad expr & \rightarrow \mem(t, i) \quad op \quad  expr\\
\end{array}
\]


\subsubsection*{Verdict at $t$}
\[
resolve(\sys_t, \mem, verdict) =  \twopartdef{verdict(q)} {\exists \tuple{q, expr}  \in I_t : eval(expr, \mem) = true }
				{?}
\]

\subsection{Algorithm}


Setup: run $net(\varphi)$ to generate the network, convert each cell to a monitor.

Let $t$ denote the timestamp $i$ the ID of the monitor.\\

\begin{itemize}
%	\item Receive $kill$ message
%		\begin{itemize}
%			\item Terminate
%		\end{itemize}
%	\item Receive observation $\sigma$
%		\begin{enumerate}
%			\item $update(\sigma, t, Q^i, \delta^i, \mem^i, \sys^i)$
%			\item $checkVerdict(\sys^i, \mem^i, verdict^i, ref^i, r^i, q_0)$
%		\end{enumerate}
%	\item Receive verdict $\tuple{t', j, v}$
%		\begin{enumerate}
%			\item $\mem^i(t', j) := v$
%			\item $checkVerdict(\sys^i, \mem^i, verdict^i, ref^i, r^i, q_0)$
%		\end{enumerate}
	\item Receive $kill(x,y)$ message:
		\begin{enumerate}
			\item Suppress $x$ from $referrers(i,y)$
			\item If $referrers(i,y) = \emptyset$
				\begin{enumerate}
					\item Supress cell $(i,y)$
					\item Send a kill $(u,v)$ message to each $(u,v) \in referents(i,y)$
					\item Set $referents(i,y)$ to $\emptyset$
				\end{enumerate}
		\end{enumerate}
	\item Receive Observation $\sigma$
		\begin{enumerate}
			\item $update(\sigma, t, Q^i, \delta^i, \mem^i, \sys^i)$
			\item $checkVerdict(\sys^i, \mem^i, verdict^i, ref^i, r^i, q_0)$
		\end{enumerate}
	\item Receive verdict $\tuple{t', j, v}$
		\begin{enumerate}
			\item $\mem^i(t', j) := v$
			\item $checkVerdict(\sys^i, \mem^i, verdict^i, ref^i, r^i, q_0)$
		\end{enumerate}
\end{itemize}

\jump
 $checkVerdict(\sys^i, \mem^i, verdict^i, ref^i, r^i, q_0): $ for $k = 0 \hdots t$
\begin{itemize}
	\item Let $v = resolve(\sys_k^i, \mem^i, verdict^i)$
	\item If  $v \neq ?$
		\begin{enumerate}
			\item Send  verdict$\tuple{k, i, v}$ to all $Mon \in ref^i$
			\item \begin{itemize}
					\item If $r^i = true$ : Set $I_k := \tuple{q_0, true}$
					\item Otherwise: terminate
			\end{itemize}
		\end{enumerate}
\end{itemize}




==> tikz/alg-orch.tex <==
\begin{tikzpicture}[aut,scale=1]
	\node[location] (m0q0) at (0,0) {$m_0,q_0$};
	\node[location, accept, right=1.5 of m0q0] (m0q1) {$m_0,q_1$};

	\tconnectt{m0q0}{m0q1}{$\MONID_1\land \neg\MONID_2$}{m0t1}{yshift=0.2cm}
	\tconnectt[bend left]{m0q0}{m0q1}{$\MONID_1 \land \MONID_2$}{m0t2}{yshift=-0.8cm}
	\tconnectt[bend right]{m0q0}{m0q1}{$\neg \MONID_1\land \MONID_2$}{m0t3}{yshift=-0.7cm}
	\tconnectt[loop left]{m0q0}{m0q0}{$\neg \MONID_1 \land \neg \MONID_2$}{m0t4}{xshift=0.5cm, yshift=+0.35cm}
	\tconnectt[loop right]{m0q1}{m0q1}{$\mathtt{t}$}{m0t5}{xshift=-.3cm}

	\node[location] (m1q0) at (4.0,0) {$m_1,q_0$};
	\node[location, accept, right=1 of m1q0] (m1q1) {$m_1,q_1$};
	\node[location, reject, below=.2 of m1q1] (m1q2) {$m_1,q_2$};

	\tconnect{m1q0}{m1q1}{$a_0$}{m1t1}
	\tconnectt{m1q0}{m1q2}{$\neg a_0$}{m1t2}{yshift=-0.2cm}
	\tconnectt[loop right]{m1q1}{m1q1}{$\mathtt{t}$}{m1t3}{xshift=-.3cm}
	\tconnectt[loop right]{m1q2}{m1q2}{$\mathtt{t}$}{m1t4}{xshift=-.3cm}


	\node[location] (m2q0) at (7.5,0) {$m_2,q_0$};
	\node[location, accept, right=1 of m2q0] (m2q1) {$m_2,q_1$};
	\node[location, reject, below=.2 of m2q1] (m2q2) {$m_2,q_2$};

	\tconnect{m2q0}{m2q1}{$b_0$}{m2t1}
	\tconnectt{m2q0}{m2q2}{$\neg b_0$}{m2t2}{yshift=-.2cm}
	\tconnectt[loop right]{m2q1}{m2q1}{$\mathtt{t}$}{m1t3}{xshift=-.3cm}
	\tconnectt[loop right]{m2q2}{m2q2}{$\mathtt{t}$}{m1t4}{xshift=-.3cm}
%	\tconnect{q0}{q1}{$a \lor b$}{t1}
%	\tconnect[loop right]{q1}{q1}{$\vt$}{t2}
%	\tconnect[loop left]{q0}{q0}{$\neg a \land \neg b$}{t2}
\end{tikzpicture}


==> title-acm.tex <==

%
\title
[On the Monitoring of Decentralized Specifications]%
{On the Monitoring of Decentralized Specifications:\\ Semantics, Properties, Analysis, and Simulation
}%



%\author{
%  ANTOINE EL-HOKAYEM and YLI\`ES FALCONE
%  \affil{, \\ F-38000 Grenoble, France}


  \author{Antoine El-Hokayem}
  \orcid{0000-0003-2925-0540}
  \affiliation{%
    \institution{Univ. Grenoble Alpes, CNRS, Inria, Grenoble INP, LIG}
    \streetaddress{}
    \city{F-38000 Grenoble}
    \country{France}}
  \email{antoine.el-hokayem@univ-grenoble-alpes.fr}

  \author{Yli\`es Falcone}
  \affiliation{%
    \institution{Univ. Grenoble Alpes, CNRS, Inria, Grenoble INP, LIG}
    \streetaddress{}
    \city{F-38000 Grenoble}
    \country{France}}
  \email{ylies.falcone@univ-grenoble-alpes.fr}



  %\setcopyright{none}  

  \keywords{Runtime Verification, Monitoring, Simulation, Decentralized Monitoring, Automata, Eventual Consistency}


==> to-append.tex <==


\paragraph{Necessary Conditions for Monitoring.}
A general decentralized monitoring algorithm requires the following the conditions to reach a similar verdict than a centralized monitoring algorithm.
\begin{proposition} \label{prop:equiv}
\todo{Reformulate}
Consider a centralized automaton $\aut$, and an equivalent decentralized automaton with a root monitor $\aut_0$.
We have $\verdictf_\aut(\Delta_{\aut}^*(q_{0_\aut}, \rho)) = \verdictf_{\aut_0}(q_{0_{\aut_0}}, \rho)$ iff:
\begin{enumerate}
	\item $\aut$ and $\aut_0$ are monitorable
	\item All monitors communicate eventually (within a fixed delay) 
\end{enumerate}
\end{proposition}



\begin{proof}[Proof of \rprop{prop:equiv}] 
\todo{Sketch}
	(1) is for the termination of $\Delta*$\\
	(2) is to map the monitor id to the verdict (the verdict must be received)
\end{proof}


\paragraph{Assumptions.}
In this paper, we focus on splitting the computation from communication following the Bulk Synchronous Parallel (BSP) model~\cite{Valiant90}.
Thus, the monitoring phase consists in all monitors executing computation based on their observations, then, all of them communicating, and finally a synchronization.
For setting up the algorithms, we consider that the monitor network is a directed graph $\tuple{N, E}$ where $N$ contains all monitors and $E$ represents the edges between the monitors.
For simplicity, we assume that edges are all of equal weight, and messages transmitted from one monitor are accessible for other monitors at the next timestamp. 
Additionally, for input specification we use LTL that is converted into monitor automata.
We do not elaborate on the generation of automata from the LTL formulae nor simplification of boolean and LTL formulae. 
The generation of the deterministic automata is done using \texttt{$\mathtt{LTL_3}$ Tools}~\cite{LTL3Tools} and simplification is done using \texttt{ltlfilt} from \texttt{Spot}~\cite{Spot}. 



